Asynchronous Federated Learning with Reduced Number of Rounds and with Differential Privacy from Less Aggregated Gaussian Noise

The feasibility of federated learning is highly constrained by the server-clients infrastructure in terms of network communication. Most newly launched smartphones and IoT devices are equipped with GPUs or sufficient computing hardware to run powerful AI models. However, in case of the original synchronous federated learning, client devices suffer waiting times and regular communication between clients and server is required. This implies more sensitivity to local model training times and irregular or missed updates, hence, less or limited scalability to large numbers of clients and convergence rates measured in real time will suffer. We propose a new algorithm for asynchronous federated learning which eliminates waiting times and reduces overall network communication - we provide rigorous theoretical analysis for strongly convex objective functions and provide simulation results. By adding Gaussian noise we show how our algorithm can be made differentially private -- new theorems show how the aggregated added Gaussian noise is significantly reduced.

==> Section/02_Relatedwork.tex <==
\section{Related Work}

% \subsection{Definition of Federated Learning Formulation}

We assume there are $K$ clients over which the data is partitioned, with $\mathscr{D}_{k}$ \footnote{In FL setting, the data distribution could be IID or non-IID and may have unbalanced property.} is the set of indexes of data points on client $k$ and the number of available samples on client $k$ is $n_k = \lvert{\ \mathscr{D}_k}\rvert$. A federated learning system is a learning process where the total $K$ clients collaboratively train a global model $w$ and client $k$ does not exchange its own local data $\mathscr{D}_k$ to other clients or server. In particular, the goal is typically to minimize the following objective function \cite{mcmahan,chen2019fedhealth}:
\begin{equation}
    \min_{w \in \mathbb{R}^{d}}{F(w)} = \sum_{k=1}^{K} \frac{n_k}{n} F_k(w)\label{eq6}
\end{equation}
with $F_{k}$ is the local loss function in client $k$, specifically:
\begin{equation}
F_{k}(w) = \frac{1}{n_k} \sum_{i \in \mathscr{D}_k} f_i(w)
\end{equation}
From the perspective of accuracy \cite{yang2019federated}, we define $\mathscr{D} = \mathscr{D}_1 \cup \mathscr{D}_2 ... \cup \mathscr{D}_K$ and the accuracy of model over $\mathscr{D}$ is $\mathscr{A}_\mathscr{D}$ and the accuracy of model using FL is $\mathscr{A}_{fl}$. Formally, we say the federated learning has $\epsilon$-accuracy if the following requirement is satisfied: $\lvert{\ \mathscr{A}_\mathscr{D} - \mathscr{A}_{fl} }\rvert < \epsilon$.

==> Section/04_Convergence_Analysis.tex <==
\section{Convergence Analysis}

\subsection{Convergence Analysis of Hogwild!}
% We will focus on an important special case of the problem, characterized by $F$ being a strongly convex function over some convex domain $\mathbb{W}$ (which is assumed to be a subset of some Hilbert space) \cite{rakhlin2011making}.

% A function $F$ is $\mathbb{L}$-smooth if it is differentiable and has Lipschitz gradients,
% \begin{align}
% \nabla F(w\;') - \nabla F(w) \leq \mathbb{L}\norm{w\;' - w}
% \end{align}
% where $\mathbb{L} > 0$ and $\forall w, w\;' \in \mathbb{R}^d$

% % http://www.rpi.edu/dept/arc/training/latex/LaTeX_symbols.pdf
% Formally, we also say that a function $F$ is $\lambda$-strongly convex, if for all $w$, $w\;'\in \mathbb{W}$ and any subgradient $g$ of $F$ at $w$,
% \begin{align}
% F(w\;') \geq F(w) + \langle g, w\;' - w \rangle  + \frac{\lambda}{2}\norm{w\;' - w}^2
% \end{align}

% We define the (unique) optimal solution of $F$ as $w^{*}$. Formally, a function $F$ is $\mu$-smooth with respect to $w^{*}$ if for all $w \in \mathbb{W}$,
% \begin{align}
% F(w) - F(w^{*}) \leq \frac{\mu}{2}\norm{w - w^{*}}^2
% \end{align}

% Such functions arise, for instance, in logistic and least squares regression, and in general for learning linear predictors where the loss function has a Lipschitz continuous gradient.

% The paper in \cite{leblond2018improved} states the theoretical results of their analysis of Hogwild! with inconsistent reads and writes in the framework.

% \theoremstyle{definition}
% \begin{definition}\label{SGDbounded}
% Let $\sigma^2$ = $\mathbb{E}$ $\norm{f_{i}\;' (w^{*})}^2$ be the variance of the gradient estimator at the optimum. The classical theoretical analysis of SGD assumes that the stochastic gradients are uniformly bounded, i.e. there exists a finite (fixed) constant $\sigma < \infty$, such that:
% $\mathbb{E} \norm{\nabla F(w)}^2 \leq \sigma^2$ \cite{nguyen2018sgd}.

% \end{definition}

% For reference, we start by giving the rate of convergence of serial SGD \cite{schmidt2014convergence}.

% \theoremstyle{definition}
% \begin{definition}
% As in \cite{recht}, we introduce $\triangle_{r} := \max_{v \in (1..d)}$ $|$ ${i:v \in S_{i}} |$. $\triangle_{r}$ is the maximum right-degree in the bipartite graph of the factors and the dimensions, i.e., the maximum number of data points with a specific feature. For succinctness, we also define $\triangle := \frac{\triangle_{r}}{n}$. We have $1 \leq \triangle{r} \leq n$, and hence $\frac{1}{n} \leq \triangle \leq 1$.
% \end{definition}

% \begin{assumption}{\textbf{(bounded overlaps)}}
% We assume that there exists a uniform bound, called $\tau$, on the maximum number of iterations that can overlap together. We say that iterations $r$ and $t$ overlap if at some points they are processed concurrently. One iteration is being processed from the start of the reading of the shared parameters to the end of the writing of its update. The bound $ \tau$ means that iterations $r$ cannot overlap with iteration $t$ for $r \geq t + \tau + 1$, and thus that every coordinate update from iteration $t$ is successfully written to memory before the iteration $t + \tau + 1$ starts.
% \end{assumption}

% \theoremstyle{definition}
% \begin{theorem}{\textbf{Convergence guarantee and rate of SGD}}
% Let a $\leq$ $\frac{1}{2}$. Then  for any step size $\gamma = \frac{a}{\mathbb{L}}$, SGD converges in expectation to $b$-accuracy at a geometric rate of at least: $\rho(a) = \frac{a}{\kappa}$, i.e, $\mathbb{E}$ $\norm{x_{t} - x^{*}}^2 \leq (1 - \rho)^{t} \norm{x_{t} - x^{*}}^2$ + $b$ with $b = 2\frac{\gamma \sigma^2}{\mu}$ and satisfies $\mu$-strong requirement.
% \end{theorem}

% As SGD only converges linearly up to a ball around the optimum, to make sure we reach $\epsilon$-accuracy, it is necessary that $2\frac{\gamma \sigma^2}{\mu} \leq \epsilon$, i.e, $\gamma \leq \frac{\epsilon \mu}{2 \sigma^2}$. All told, in order to get linear convergence to $\epsilon$-accuracy, serial SGD requires $\gamma \leq \min\{\frac{1}{2 \mathbb{L}},\frac{\epsilon \mu}{2 \sigma^2}\}$

% We define the update $gt_t := g(\hat{x}_t,\hat{\alpha}_t,i_t)$, is an unbiased estimator of the true gradient at $\hat{x}_t$ in conditional expectation. For all $t > 0$,

% $a_{t+1} \leq (1 - \frac{\gamma \mu}{2}) a_t + \gamma^2 C_1 \mathbb{E} \norm{g_t}^2 + \gamma^2 C_2 \sum_{u=t-\tau}^{t-1} \mathbb{E}\norm{g_u}^2 + 2\gamma e_t$,
% where $C_1 := 1 + \sqrt{\triangle_{r}}$ and $C_2 := \sqrt{\triangle} + \gamma \mu C_1$.

% \theoremstyle{definition}
% \begin{theorem}{\textbf{Convergence guarantee and rate of Hogwild!}}\label{Hogwild}
% Let $a^{*}(\tau) := $ $\frac{1}{5(1 + 2\tau\sqrt{\triangle}) \xi(\kappa, \triangle, \mathbb{T})}$ where $\xi(\kappa, \triangle, \mathbb{T}) := \sqrt{1 + \frac{1}{2 \kappa} \min(\frac{1}{\sqrt{\triangle}}}, \tau)$, note that $\xi(\kappa, \triangle, \mathbb{T}) \approx 1$ unless $\kappa < \frac{1}{\sqrt{\triangle}} (\leq \sqrt{n})$.

% For any step size $\gamma = \frac{a}{\mathbb{L}}$ with $a < \min\{a^{*}(\tau), \frac{\kappa}{\tau}\}$, the inconsistent read iterates of $Algorithm$ 1 converge in expectation to $b$-accuracy at a geometric rate of at least: $\rho(a) = \frac{a}{\kappa}$, i.e, $\mathbb{E}$ $\norm{x_{t} - x^{*}}^2 \leq (1 - \rho)^{t} (2\norm{x_{0} - x^{*}}^2$) + $b$, where we define $b = \epsilon^{2}(\frac{8\gamma(C_{1} + \tau C_{2})}{\mu} + 4 \gamma^{2} C_{1}\tau)$ and and $C_1$ and $C_2(\gamma)$ are defined above.
% \end{theorem}

% Once again this result is quite close to the one obtained for serial SGD. Note that we recover this exact condition (up to a small constant factor) if we set $\tau = 0$, i.e. if we force our asynchronous algorithm to be serial.

% \begin{corollary}[\textbf{Speedup condition}]
% Suppose $\tau = \mathcal{O}(\min\{\frac{1}{\sqrt{\triangle}},\kappa\})$. Then for any step size $\gamma \leq \frac{a^{*}(\tau)}{\mathbb{L}} = \mathcal{O}(\frac{1}{\mathbb{L}})$ (i.e., any allowable step size for SGD), Hogwild! converges geometrically to a ball of radius $r_h = \mathcal{O}(\frac{\gamma \sigma^2}{\mu})$ with rate factor $\rho = \frac{\gamma \mu}{2}$ (similar to SGD), and is thus linearly faster than its sequential counterpart up to a constant factor.

% Moreover, a universal step size of $\Theta(\frac{1}{\mathbb{L}})$ can be used for Hogwild! to be adaptive to local strong convexity with a similar rate to SGD (i.e., knowledge of $\kappa$ is not required).
% \end{corollary}

% If $\gamma = \mathcal{O}(\frac{1}{\mathbb{L}})$, Hogwild! obtains the same convergence rate as SGD and converges to a ball of equivalent radius. Since the maximum step size guaranteeing linear convergence for SGD is also $\mathcal{O}(\frac{1}{\mathbb{L}})$, Hogwild! is linearly faster than SGD for any reasonable step size – under the condition that $\tau = \mathcal{O}(\min\{\frac{1}{\sqrt{\triangle}},\kappa\})$. We also remark that since $\gamma \leq \frac{1}{\mathbb{L}}$ and $\tau \leq \kappa$, we have $\gamma \mu \tau \leq 1$, which means the condition $a \leq \frac{\kappa}{\mu}$ is superseded by $a \leq a^{*}(\tau)$ in $\ref{Hogwild}$.

% The papers in \cite{leblond2018improved,mania2017perturbed} noted that our results are derived directly on iterates, that is, we bound the distance between $x_t$ and $x^{∗}$. We can easily obtain results on function values to bound $\mathbb{E}[f(x_t) - f(x^*)]$ by adapting the classical smoothness inequality: $\mathbb{E}[f(x_t) - f(x^*)] \leq \mathbb{E}\norm{x_t - x^*}^2$ to the asynchronous parallel setting.

% \textbf{Convergence to $\epsilon$-accuracy.}
% As noted in \cite{mania2017perturbed}, for our algorithm to converge to $\epsilon$-accuracy for some $\epsilon > 0$, we require an additional bound on the step size to make sure that the radius of the ball to which we converge is small enough. For SGD, this means using a step size $\gamma = \mathcal{O}(\frac{\epsilon \mu}{\sigma^2})$. We can also prove that under the conditions that $\tau = \mathcal{O}(\frac{1}{\sqrt{\triangle}})$ and $\gamma \mu \tau \leq 1$, Hogwild! requires the same bound on the step size to converge to $\epsilon$-accuracy. If $\epsilon$ is small enough, the active upper bound on the step size is $\gamma = \mathcal{O}(\frac{\epsilon \mu}{\sigma^2})$ for both algorithms. In this regime, we obtain a relaxed condition on τ for a linear speedup. The condition $\tau \leq \kappa$ which came from comparing maximum allowable step sizes is removed. Instead, we enforce $\gamma \mu \tau \leq 1$, which gives us the weaker condition $\tau = \mathcal{O}(\frac{\sigma^2}{\epsilon \mu^2})$. Our condition on the overlap is then: $\tau = \mathcal{O}(\min\{\frac{1}{\sqrt{\triangle}},\frac{\sigma^2}{\epsilon \mu^2}\})$. We see that this is similar to the condition obtained in \cite{mania2017perturbed} in their Hogwild! analysis, although we have the variance at the optimum $\sigma^2$ instead of a squared global bound on the gradient.

% Moreover, the paper in \cite{nguyen2018sgd} shows that for stochastic problems arising in machine learning such bound always holds in $\ref{SGDbounded}$. They also propose an alternative convergence analysis of SGD with diminishing learning rate regime, which results in more relaxed conditions than those in \cite{bottou2018optimization}, specifically their work extends the analysis of SGD to provide analysis of Hogwild! with diminishing step sizes and without the assumption on bounded gradients.

% \subsection{Convergence Analysis of Averaging Federated learning}
% Federated Averaging \cite{sahu2018convergence,doan2017convergence,wang2019adaptive} is stochastic algorithms by nature; in that, each step of these algorithms, only a fraction of the users are sampled to perform the update. Moreover, the local optimizer could be stochastic, e.g. SGD. It is well known that for stochastic methods in order to converge to a stationary point, a decreasing step-size is required. This is in contrast to the non-stochastic methods, e.g. gradient descent, that can find a stationary point with constant step size. In order to analyze the convergence behavior of such methods with constant step size, which is what is usually deployed in practice, we need to somehow control the dissimilarity among the local functions. This could be achieved through assuming IID, i.e. homogeneous, data among users. But we aim to generalize this idea to heterogeneous setting, which would better represent the federated learning.


% \subsection{Convergence Analysis of Hybrid system}

==> Section/05_Experiment.tex <==
\section{Experiment}
\label{sec:experiment}

Without loss of generality, we implement SGD and Hogwild! algorithms with constant step sizes. Moreover, it is sufficient to only consider our $k$-round asynchronous FL where the clients run SGD with constant step sizes because this is the most practical setup. We use Python and Tensorflow in our programming. 

\textcolor{red}{Ha to Nhuong: need to describe everything in detail. For example, how many samples in the training datasets. What is the configuration of clients and system. How do you implement Hogwild!, i.e., how to implement the memory lock for atomic reads and writes. What is the delay we introduce for atomic reads/ writes in the simulation.}

In this paper, we mainly focus on convex problem in machine learning, especially logistic regression problem with $\ell_{2}$ regularization.

The weight $w$ of the logistic function can be learned by minimizing the log-likelihood function $J$ (the logistic regression loss function) through gradient descent.
\begin{equation} \label{eq_logstic_reg}
    J = - \sum_{i}^N [ y_{i} \cdot \log (\sigma_i) + (1 - y_{i}) \cdot \log (1 - \sigma_i) ] + \frac{\lambda}{2}\norm{w}^{2},
\end{equation}
where $N$ is the number of training samples, $\lambda$ is regularization parameter, $\sigma$ is a sigmoid function with parameters weight $w$, bias value $b$ and input data $x$ defined as:
\begin{equation} \label{eq_sigmoid}
    \sigma(w, x, b) = \frac{1}{1 + e^{-(w^{\mathrm{T}}x + b)}}.
\end{equation}

\subsection{Simulation of SGD and Hogwild! and their comparison}
\label{subsec:hogwild_simu}

We consider the binary classification for digits $0$ and $1$ for MNIST dataset. The goal of this experiment is to study the behavior of Hogwild! and the limitation of delay variable $\tau$. \textcolor{red}{For simulating the atomic read and write operation, we partition the full model $w$ into $m$ parts and these parts are locked by synchronized lock to guarantee the atomic operation. Moreover, in order to simulate the delay of read and write operation, we define atomic read and write operation will take 2 milliseconds, 1 millisecond respectively.} The detail sett up of the experiments is described below:
\begin{table}[ht]
\caption{Hogwild! training parameters}
\label{tbl_hogwild}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule

Regularization parameter $\lambda$   & 1/$N$ &    \\
Learning rate $\eta$ & 0.001 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
%Size of Dataset & ????&   \\

% \hline
Number of atomic writes & 50000 &                       \\
% \hline
Image size & 28x28   & grayscale                        \\
Data set records $N$ & 14867 &                          \\
% \hline
Number of threads $n$ & 1/3/5/10/15/20 &                  \\
% \hline
Number of masks $m$ & 14 &                               \\
% \hline
Epoch & 20 &                                            \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[hbt]
  \centering
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{tikz/04_hogwild_and_sgd_train_loss.PNG}
\caption{The training loss at the end of each epoch.}
\label{fig:hogwild_train_err}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{tikz/03_hogwild_and_sgd_train_duration.PNG}
\caption{Average training duration with different number of threads.}
\label{fig:hogwild_duation}
  \end{minipage}
\end{figure}

Figures~\ref{fig:hogwild_train_err} and \ref{fig:hogwild_duation} show the training error and speedup rate for training process using the Hogwild! algorithm. When n$\_$thread=1, Hogwild! is exactly SGD. As can be seen from Figure~\ref{fig:hogwild_train_err}, while the number of threads increases, the values of training error for all threads are nearly the same. It means that single thread SGD and Hogwild! with multiple threads have the same accuracy or training error. In contrast to Figure~\ref{fig:hogwild_train_err}, we see a significant decrease of training duration when the number of threads goes up. However, the number of joined threads needs to be reasonable due to the limit of max delay $\tau$ and the number of masks, which can reduce the performance of training process due to the effect of collision in atomic read and atomic write constraints. For example, when n$\_$thread=20, the duration increases instead of decreasing due to the effect of atomic read or write. 

\subsection{Simulation of our $k$-round asynchronous FL}
\label{subsec:kroundFL_simu}

In order to understand the behavior of the FL systems. We conduct the following experiments. 


\begin{table}[ht]
\caption{Federated Learning with different number of samples.}
\label{tbl_samples}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.001 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
% \hline
Number of clients $n$ & 3 &                              \\
% \hline
Image size & 28x28   & grayscale                    \\
Train dataset records & 14867 &                          \\

% \hline
Number of samples $s$ & 10/50/100/500/1K/2K/\\ &2.5K/10K/15K &                  \\
% \hline
Number of round $r$ & 5 &                               \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_sample_train_error.PNG}
\caption{FL with different number of samples.}
\label{fig:fl_sample}
\end{figure}

\vspace{0.2cm}
\noindent
\textbf{Varying the size of samples $s$ while fixing parameters $k,n$ and $\eta$:} The goal of this experiment is that $s$ can not be arbitrary large due to the restriction from the delay parameter $\tau$. To make the analysis simple, we consider $1$-round asynchronous FL (i.e., original FL). The detailed setup of this experiment for logistic regression problem is described in Table~\ref{tbl_samples}.

Figure~\ref{fig:fl_sample} reveals that when the number of samples $s=500$, we gain the highest accuracy. In addition, if we continue to increase the number of samples, the accuracy keeps nearly unchanged, i.e, large number of samples does not guarantee the improvement of accuracy.

\vspace{0.2cm}
\noindent
\textbf{Varying the number of clients $n$ while fixing parameters $k,s$ and $\eta$:} The goal of this experiment is that $n$ can not be arbitrary large due to the restriction from the delay parameter $\tau$. To make the analysis simple, we consider $1$-round asynchronous FL (i.e., original FL). \textcolor{red}{We choose the small stepsize for the simulation due to the fact that we need the large number of samples and clients to show that large number of clients can affect the train accuracy.} The detail parameters of this experiment are illustrated in Table~\ref{tbl_clients}.

\begin{table}[ht]
\caption{Federated Learning with different number of clients.}
\label{tbl_clients}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.00025 &  fixed                       \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                \\
% \hline
% \hline
Image size & 28x28   & grayscale                    \\
Data set records & 14867 &                          \\
% \hline
Number of clients $n$ & 5/10/20/30/40/50 &                  \\
Number of samples $s$ & 5000 &                  \\
% \hline
$k$-round & 5 &                               \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_client.PNG}
\caption{FL with different number of clients.}
\label{fig:fl_client}
\end{figure}

Figure~\ref{fig:fl_client} shows that when number of client $n=30$, the training process gain the lowest train error, i.e, the largest accuracy while if $n$ continue to increase, the accuracy will dramatically decreases.

\vspace{0.2cm}
\noindent
\textbf{Varying the round parameter $k$ while fixing parameters $n,s$ and $\eta$:} The goal of this experiment is to verify the convergence rate of the system when $k$ increases. Table~\ref{tbl_k_round} defines the detail parameters of the experiment.


\begin{table}[ht]
\caption{Federated Learning with different number of $k$-round.}
\label{tbl_k_round}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule
Learning rate $\eta$ & 0.0001 &  fixed                         \\ 
% \hline
Data set & MNIST & $0$ and $1$ digit                    \\
% \hline
% \hline
Image size & 28x28   & grayscale                        \\
Data set records & 14867 &                              \\
% \hline
Number of clients $n$ & 3 &                                  \\
Number of samples $s$ & 1000 &                              \\
% \hline
Number of rounds & 5 &                                   \\
$k$-round & 1/2/3/4/5/6 & asyn-round of client                   \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{tikz/01_fl_vary_k_round.PNG}
\caption{FL with different number of $k$-round.}
\label{fig:fl_k_round}
\end{figure}

As can be seen from Figure~\ref{fig:fl_k_round}, when we change the $k$-round value from 1 to 2 and 3, the train error goes down dramatically. It means that asynchronous FL helps the model converge faster than the traditional FL. However, when we continue to increase the value $k$, the train error almost remains unchanged.


\textcolor{red}{\textbf{Important Note}:} From the implementation, we have the following observation: assume that there exists a good $k$-asynchronous FL, i.e., the clients always get a new model $w$ from the server before finishing all $k$ rounds of computation. Then for any $k'(>k)$-round asynchronous FL, it should include that good $k$-round asynchronous one. This fact leads to the important following result: the clients always get the new model $w$ before finishing all $k$ rounds rather than $k'$ rounds. In other words, $k'$ can be arbitrary large or the clients seem never be in \textit{waiting mode} as described in Figure~\ref{fig:framework_waiting}. Therefore, the designer only needs to find the optimal numbers $s$ and $n$ and can ignore the parameter $k$ by setting it  large. This allows the clients and server to work in a fully asynchronous mode. 


\subsection{Real applications of Federated learning}

\textbf{Text prediction on Android phone}: We can create an Android phone for chatting purpose. Based on the text content from client, we can used it for training a text prediction model. We can take reference from Google Keyboard application \cite{GoogleAIBlog,hard2018federated}.

\textbf{Diseases Detection based on daily activities}: Based on mobile phone, we can collect behavioral data from client, for example, sleep time, exercise habit, daily activities. Certain activities in daily life can reflect early signals of some diseases, so we can create a mode for detecting common diseases. For example, without enough sleep, people can suffer from seizure or mental disorders \cite{chen2019fedhealth}.

\textbf{Music recommendation engine:} which recommends music on an app for users. Specifically, we can predict emoji from text typed on a mobile keyboard and then recommends appropriate music for users \cite{ramaswamy2019federated}.

\textbf{Fraud detection model:} multiple banks could train a common powerful fraud detection model without sharing their sensitive customer data with each other through Federated Learning.


\textcolor{red}{https://hackernoon.com/a-beginners-guide-to-federated-learning-b29e29ba65cf}


\textbf{Technologies and Frameworks for Federated Learning
:} Some of the popular and recent Federated Learning frameworks include TensorFlow Federated, an open source framework by Google for experimenting with machine learning and other computations on decentralized data. PySyft is a open source library that is built on top of PyTorch for encrypted, privacy preserving deep learning. Federated AI Technology Enabler (FATE) is an open-source project initiated by Webank’s AI group to provide a secure computing framework to support the Federated AI ecosystem.

Several new startups such as S20.ai, Owkin, and Snips have emerged in this space creating new tools and enterprise solutions around Federated Learning and other secure computation techniques across different verticals

\textbf{Federated Learning is still in its early stages and faces numerous challenges with its design and deployment.
}
For instance, its feasibility is highly constrained by the capabilities of the edge devices to perform local training and inferencing. While this may not remain a major barrier to entry as most smartphones and IoT devices newly launched are equipped with GPUs or sufficient computing hardware to run powerful AI models. Today it’s still impossible to train a network without compromising device performance and user experience or compressing a model and resorting to a lower accuracy.

Local training of supervised models requires labeled data which isn’t available or difficult to produce in most cases. A good way to tackle this challenge is by defining the Federated Learning problem and designing data pipeline such that labels are captured in an implicit way, for example, user’s interactions, feedback on model responses based on certain actions taken or events triggered, etc.

In real world cases, model convergence time is higher in the Federated setup as compared to the traditional central training approach. There could be reliability issues where not all devices participate in the Federated Learning process due to connectivity issues, different app usage patterns and model training times, irregular or missed updates, etc. Federated Learning should be considered only when the size of the data and cost of aggregating from distributed sources is very high. inconsistent model versions across the clients does not affect the experience too much for a significant time window and the central model can converge with minimal client participation.

Finally, the mindset of centrally aggregating data and creating silos by large companies for competitive advantage would be a major challenge to drive the adoption of Federated Learning. Effective data protection policies and appropriate incentives and business models around decentralizing data can tackle these issues and develop the Federated AI ecosystem
















==> Section/08_Proposal_citations.tex <==
\section{Proposal Citations}
\label{sec:proposal_citations}

The detail list of papers in federated learning is illustrated in ~\cite{yang2019federated,tianli2019federated}.

Ref: https://arxiv.org/pdf/1902.04885.pdf

Ref: https://arxiv.org/pdf/1908.07873.pdf

\vspace{2mm}
\noindent
\textbf{Introduction of Federated Learning}

~\cite{konevcny2016federated} introduced the concept of federated learning in 2016. They used the android application (Google keyboard) to demonstrate the text prediction application.

~\cite{mcmahan} described the original federated learning for deep learning task. Specifically, the server will take average of all models from clients.

~\cite{tianli2019hetero} introduced FedProx, which makes a small modification to the~\cite{mcmahan} method to help ensure convergence, both theoretically and in practice. FedProx can also be interpreted as a generalized, reparameterized version of FedAvg that has practical ramifications in the context of accounting for systems heterogeneity across devices.

\vspace{2mm}
\noindent
\textbf{Architecture of Federated Learning}

\begin{figure}[ht]
  \centering
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{Figures/horizon.PNG}
\caption{Horizontal architecture of FL.}
\label{fig:horizontal_fl}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\textwidth}
 \includegraphics[width=\columnwidth,keepaspectratio]{Figures/vertical.PNG}
\caption{Vertical architecture of FL.}
\label{fig:vertical_fl}
  \end{minipage}
\end{figure}

\textbf{Horizontal Federated Learning or sample-based federated learning} \cite{mcmahan,tianli2019hetero,bonawitz2019towards,konevcny2016federated,konevcny2016federated_com}, is applied in the scenarios that local data sets in clients share the same feature space but different in samples. A typical architecture for a horizontal federated learning system is shown in Figure ~\ref{fig:horizontal_fl}. In this system, $k$ clients with the same data structure collaboratively train independently global model with the help of a parameter server. In addition, a typical assumption \cite{phong2018privacy} is that the participants are honest while the server is honest-but-curious, hence no leak information from any participants to other participants and the server is allowed.

\textbf{Vertical federated learning or feature-based federated learning} \cite{nock2018entity,yang2019federated,hardy2017private} is applied in cases that data sets in client sides share the same sample space but differ in feature space (shown in Figure~$\ref{fig:vertical_fl}$a). It is the process of aggregating these different features and computing the training loss and gradients in a privacy-preserving manner to build a model with data from parties collaboratively. In addition, a vertical federated learning system typically assumes honest-but-curious participants. In the security perspective, it means that the adversary can only learn data from the corrupted clients but not data from other clients or from server. Recently, there are a lot of researches which have proved that FL can work very well with various machine learning models (for example, logistic regression, tree structure and neural network) \cite{gascon2016secure,karr2009privacy,vaidya2002privacy,wan2007privacy}.

\textbf{Federated Transfer Learning} \cite{pan2009survey} can be used to the scenarios that the data sets in client sides are different from in both sample spaces and feature space, so transfer learning technique can handle the problem of lacking data (few samples and features) or weak supervision (few labels). We can distinguish the major difference between vertical FL and federated transfer learning is that federated transfer learning can exchange models among clients, which is not seen in vertical FL (shown in Figure~$\ref{fig:vertical_fl}$a,b). However, the set of overlapped data from clients could be small (for example the different businesses in reality) and make federated transfer learning less attractive and effective. Interestingly, the paper in \cite{yang2018secureftl} proposes a possible solution to these above challenges by exchanging the models using homomorphic encryption among clients, which leverages the transfer learning technique proposed by \cite{pan2009survey} to provide solution for training FL with the sample and feature space under a data federation and privacy-preserving constraints.

\vspace{2mm}
\noindent
\textbf{Privacy-preserving and Security under Federated Learning}

\textbf{Privacy} is one of the essential properties of federated learning. This requires security models and analysis to provide meaningful privacy guarantees.

Secure Multi-party Computation (SMC) \cite{wenliang,payman,dan} naturally involved multiple parties, and provide security proof in a well-defined simulation framework to guarantee complete zero knowledge, that is, each party knows nothing except its input and output. Zero knowledge is very desirable, but this desired property usually requires complicated computation protocols and may not be achieved efficiently.


Differential Privacy \cite{cynthia,dwork2014algorithmic,abadi2016deep,geyer2017differentially,mcmahan2017learning} involves in adding noise to the data, or using generalization methods to obscure certain sensitive attributes until the third party cannot distinguish the individual, thereby making the data impossible to be restore to protect user privacy. However, the root of these methods still require that the data are transmitted elsewhere and these work usually involve a trade-off between accuracy and privacy.

Homomorphic Encryption \cite{rivest,qingchen,abbas} is also adopted to protect user data privacy through parameter exchange under the encryption mechanism during machine learning. Unlike differential privacy protection, the data and the model itself are not transmitted, nor can they be guessed by the other party’s data. Therefore, there is little possibility of leakage at the raw data level. Recent works adopted homomorphic encryption for centralizing and training data on cloud.

\textbf{Model-poisoning attacks in Federated Learning}

~\cite{nasr2019comprehensive} shows how adversarial participants, in the federated learning setting, can successfully run active membership inference attacks against other participants, even when the global model achieves high prediction accuracies.

~\cite{eugene} argued that federated learning is fundamentally vulnerable to backdoor attacks. First, when training with millions of participants (\textit{the attackers can directly influence the weights of the global model}), it is impossible to ensure that none of them are malicious. Second, federated learning by design has no visibility into what these participants are doing locally (\textit{the attackers can train the global model in any way that benefits poisoning}), and “secure aggregation” provably prevents anyone from auditing participants’ updates to the joint model. Existing defenses against data poisoning cannot be used for federated learning because they all require access to the training data.

~\cite{arjun} exploited the lack of transparency in the agent updates, and explore the possibility of an adversary controlling a small number of malicious agents performing a model poisoning attack. The adversary’s objective is to cause the jointly trained global model to misclassify a set of chosen inputs with high confidence, i.e., it seeks to poison the global model in a targeted manner. Since the attack is targeted, the adversary also attempts to ensure that the global model converges to a point with good performance on the test or validation data. Moreover, they focus on an adversary which directly performs model poisoning instead of data poisoning \cite{battista,huang} as the agents’ data is never shared with the server.


\vspace{2mm}
\noindent
\textbf{Asynchronous SGD training technique}~\cite{zinkevich2009slow,lian2015asynchronous,lian2017asynchronous,zheng2017asynchronous,meng2017asynchronous,stich2018local,shi2019distributed} is widely used in traditional distributed stochastic gradient descent (SGD). Typically, asynchronous SGD converges faster than synchronous SGD. However, classic asynchronous SGD directly sends gradients to the server after each local update, which is not practical for edge devices (such as mobile or IoT devices) due to the unreliable and slow communication.

% ~\cite{congxie2019} \textcolor{red}{proposed a new asynchronous federated optimization algorithm and proved that the proposed approach has near-linear convergence to a global optimum, for both strongly and non-strongly convex problems. However, their proof is not based on Hogwild! scheme}.

\vspace{2mm}
\noindent
\textbf{Communication Cost in Federated Learning}

In order to reduce communication in such a setting, two key aspects to consider are: (1) reducing the total number of communication rounds, or (2) reducing the size of transmitted messages at each round.

Local updating methods can reduce the total number of communication rounds \cite{jaggi2014communication,zhang2015deep,smith2016cocoa}.

Model compression schemes such as sparsification, subsampling, quantization, compression algorithms can significantly reduce the size of messages communicated at each round \cite{chen2015compressing,han2015deep_compression,konevcny2016federated_com,jacob2018quantization,caldas2018expanding, sattler2019robust}.

Decentralized training \cite{lian2017can,he2018cola,lalitha2019decentralized} and hierarchical communication \cite{lin2018don,liu2019edge} are proposed by to reduce the communication and computation from the central server. Specifically, the intermediate servers will aggregate the updates from clients and then the central server only aggregate updates from edge servers.

\vspace{2mm}
\noindent
\textbf{Fault Tolerance in Federated Learning system:}
The federated learning system in reality also needs to address not only high communication costs but also stragglers and fault tolerance issues~\cite{tandon2017gradient,bonawitz2019towards,yu2019distributed,chen2019efficient}.


\vspace{2mm}
\noindent
\textbf{Benchmark tools for federated learning system}

LEAF \cite{caldas2018leaf} is an open-source, modular benchmarking framework for learning in federated settings. Source code: https://leaf.cmu.edu/

TensorFlow Federated \cite{tensorflow_federated} is an open-source framework for machine learning and other computations on decentralized data, which is released by Tensorflow team. Source code: https://github.com/tensorflow/federated

\vspace{2mm}
\noindent
\textbf{Dataset}

MNIST~\cite{lecun-mnisthandwrittendigit-2010}

FashionMNIST~\cite{xiao2017fashion}

CIFAR-10~\cite{Krizhevskycifar10}

Netflix Prize dataset~\cite{Bennett07thenetflix}

UCI Smartphone~\cite{reyes2012human}



==> Section/09_Experiments_full.tex <==
\section{Experiments for asynchronous SGD | Hogwild! and asynchronous Federated Learning}

\subsection{Experiment problem}
The weight $w$ of the logistic function can be learned by minimizing the log-likelihood function $J$ (the logistic regression loss function)
\begin{equation} \label{eq_logstic_reg2}
    J = - \sum_{i}^N [ y_{i} \cdot \log (\sigma_i) + (1 - y_{i}) \cdot \log (1 - \sigma_i) ] + \frac{\lambda}{2}||\norm{w}||^{2},
\end{equation}
where $N$ is the number of training samples, $\lambda$ is regularization parameter, $\sigma$ is a sigmoid function with parameters weight $w$, bias value $b$ and input data $x$ defined as:
\begin{equation} \label{eq_sigmoid2}
    \sigma(w, x, b) = \frac{1}{1 + e^{-(w^{\mathrm{T}}x + b)}}.
\end{equation}

\subsection{Experiments for Hogwild!} \footnote{The experiments for Hogwild! solved the convex problem.}
For comparing the convergence of Hogwild! for constant and diminishing stepsize, there are some notes in the setting:

\begin{itemize}
    \item {use a reasonable value of $\lambda$.}
    
    \item{use a small value of $D$. For example, we use $D = 7$ for MNIST and Fashion MNIST and $D=8$ for CIFAR10 dataset.}
    
    \item {small value of constant stepsize.}
    
\end{itemize}

\begin{table}[tb]
\caption{Hogwild! training parameters}
\label{tbl_hogwild_exp}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule

Regularization parameter $\lambda$   & $0.1/0.15/0.05$ &    \\
Constant learning rate $\eta$ & 0.001 &                         \\ 
% \hline
Data set & MNIST &                \\

% \hline
Number of atomic writes & 12500 &                       \\
% \hline
Image size & 28x28   & grayscale                        \\
Batch size $b$ & 10 &                                   \\
% \hline
Number of threads $n$ & 3 &                             \\
% \hline
Number of masks $m$ & 7 &                               \\
% \hline
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Table~\ref{tbl_hogwild_exp} illustrates the detailed parameters used for conducting experiments for Hogwild! The goal of this experiments is to see the convergence of Hogwild! on different datasets. The results are described below:
\begin{figure}[ht]
\includegraphics[width=\columnwidth]{Experiments/Figure_mnist_01_mu_0x10_500x25_stepsize_0x001.png}
\caption{Hogwild! for MNIST dataset, digit 0/1}
\label{fig:hogwild_mnist_01_0}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_mnist_01_mu_0x15_500x25_stepsize_0x001.png}
\label{fig:hogwild_mnist_01_1}
\caption{Hogwild! for MNIST dataset, digit 0/1}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_mnist_01_mu_0x05_500x25_stepsize_0x001.png}
\label{fig:hogwild_mnist_01_2}
\caption{Hogwild! for MNIST dataset, digit 0/1}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_famnist_45_mu_0x10_500x25_stepsize_0x001.png}
\label{fig:hogwild_fashionmnist_45_0}
\caption{Hogwild! for FashionMNIST dataset, subset Coat/Sandal}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_famnist_45_mu_0x15_500x25_stepsize_0x001.png}
\label{fig:hogwild_fashionmnist_45_1}
\caption{Hogwild! for FashionMNIST dataset, subset Coat/Sandal}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_famnist_45_mu_0x05_500x25_stepsize_0x001.png}
\label{fig:hogwild_fashionmnist_45_2}
\caption{Hogwild! for FashionMNIST dataset, subset Coat/Sandal}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_cifar10_78_mu_0x10_500x25_stepsize_0x0001.png}
\label{fig:hogwild_cifar10_78_0}
\caption{Hogwild! for CIFAR10 dataset, subset Horse/Ship}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_cifar10_78_mu_0x15_500x25_stepsize_0x0001.png}
\label{fig:hogwild_cifar10_78_1}
\caption{Hogwild! for CIFAR10 dataset, subset Horse/Ship}
\end{figure}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{Experiments/Figure_cifar10_78_mu_0x05_500x25_stepsize_0x0001.png}
\label{fig:hogwild_cifar10_78_2}
\caption{Hogwild! for CIFAR10 dataset, subset Horse/Ship}
\end{figure}


\begin{table}[h]
\caption{Asynchronous Federated Learning (FL) parameters}
\label{tbl_FL_mnist_k_1}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Parameter & Value & Notes \\ [0.5ex]
\midrule

Regularization parameter $\lambda$   & $0.1$ &    \\
Constant learning rate $\eta$ & 0.001 &                         \\ 
% \hline
Data set & MNIST & Digit 4 and 5               \\
Data set & Fashion MNIST & Coat and Sandal               \\
%Size of Dataset & ????&   \\

% \hline
Number of atomic writes & 12500 &                       \\
% \hline
Image size & 28x28x1   &                         \\
Batch size $b$ & 10 &                                   \\
Asynchronous round $k$ & 1/2 &                          \\
% \hline
Number of client $n$ & 1 server and 2 clients &                  \\
% \hline
Number of masks $m$ & 7 &                               \\
% \hline
% Epoch & 20 &                                            \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Table~\ref{tbl_FL_mnist_k_1} illustrates the detailed parameters used for conducting experiments for asynchronous FL. The goal of this experiments is to see the accuracy of traditional FL and asynchronous FL with different communication round. The communication round $k$ means the number of times clients and server exchange their gradients (models) values and less value of $k$ means better communication costs. The results are described in Table~\ref{tbl_FL_mnist_k_1_result},\ref{tbl_FL_famnist_k_1_result} below:
\begin{table}[h]
\caption{Asynchronous Federated Learning result for MNIST}
\label{tbl_FL_mnist_k_1_result}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Experiment & Test Accuracy (\%) & Communication round\footnote{Number of rounds clients and server exchange their models.} \\ [0.5ex]
\midrule
Traditional FL\footnote{Traditional FL uses a constant stepsize.}  
& $93.717$ &   5       \\
Traditional FL   & $93.775$ &   4                   \\
Traditional FL   & $94.101$ &   3                   \\
Traditional FL   & $88.951$ &   2                   \\
Asynchronous FL ($k=1$)  & $96.496$  &   2          \\
Asynchronous FL ($k=2$)  & $95.904$  &   2          \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[h]
\caption{Asynchronous Federated Learning result for FashionMNIST}
\label{tbl_FL_famnist_k_1_result}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
Experiment & Test Accuracy (\%) & Communication round \\ [0.5ex]
\midrule

Traditional FL\footnote{Traditional FL uses a constant stepsize.}   
& $87.135$ &   5           \\

Traditional FL   & $87.435$ &   4           \\
Traditional FL   & $89.005$ &   3           \\
Traditional FL   & $92.727$ &   2           \\
Asynchronous FL ($k=1$)  & $97.675$  &   2          \\
Asynchronous FL ($k=2$)  & $94.145$  &   2          \\


\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\subsection{Experiments for asynchronous Federated Learning}

\subsection{Experiments for Differential Privacy - Federated Learning}

TODO: Experiments Description & Experiments Results

% Strongly convex case

% Plain convex case

% Non convex case
